Prospects of resolving and localising individual supermassive black hole binaries with pulsar timing arrays: the host ranking challenge

Pulsar Timing Arrays (PTAs) are soon expected to detect individually resolved supermassive black hole (SMBH) binaries, opening the possibility for multi-messenger discoveries. The biggest challenge will be to pinpoint the host galaxy in a large localisation area. We simulate realistic binary populations consistent with the gravitational wave (GW) background, projecting the PTA sensitivity for the next 0-10 years. We inject the loudest binary on top of the background and use one of the standard detection pipelines to constrain its properties. We cross-match the localisation areas with comprehensive all-sky galaxy catalogues and estimate the number of candidate hosts in the localisation area assessing, for the first time, the number of missing galaxies due to incomplete coverage. We develop a ranking system that excludes galaxies with properties inconsistent with the GW posteriors, and prioritizes the remaining galaxies for follow-up observations. We find a $\approx$21, $\approx$38 and $\approx$51 percent probability of resolving a binary in the next 0, 5 and 10 years, respectively, reduced to 0.3, 3.8 and 14.1 percent if we require potentially well-constrained localisation areas. The localisation areas span hundreds of square degrees, but shrink significantly with the addition of more data. They contain on average $\approx$190,000 early type galaxies and $\approx$40,000 active galactic nuclei, with $\approx$25,000 missing candidate hosts. Our ranking method can exclude about half of the potential hosts and efficiently rank those remaining when the galaxy catalogue provides SMBH masses and redshifts, but becomes more inefficient when we rely on apparent magnitudes.

==> extra.tex <==
In particular, these models describe the
galaxy stellar-mass as a Schechter function
\citep{Schechter76}:
\begin{equation}
    \label{eq:gsmf}
    \Psi\left(m_{\star1},z\right)=\ln(10)\Psi_0
    \left[\frac{m_{\star1}}{M_\psi}\right]^{\alpha_\psi}
    \exp\left(-\frac{m_{\star1}}{M_\psi}\right),
\end{equation}
where $m_{\star1}$ is the stellar mass of the galaxy, and
the dependence on the redshift $z$ is included in the
parametrization of $\Psi_0$:
\begin{equation}
    \label{eq:psi0}
    \log_{10}\left(\frac{\Psi_0}{{\rm Mpc}^{-3}}\right)=
    \psi_0+\psi_z\cdot z,
\end{equation}
by the one of $M_\psi$:
\begin{equation}
    \label{eq:mpsi}
    \log_{10}\left(\frac{M_\psi}{M_\odot}\right)=
    m_{\psi,0}+m_{\psi,z}\cdot z,
\end{equation}
and by the one of $\alpha_\psi$
\begin{equation}
    \label{eq:alphapsi}
    \alpha_\psi=1+\alpha_{\psi,0}+\alpha_{\psi,z}\cdot z.
\end{equation}

%----------------------------------------------------------------

We then model as power laws both the galaxy pair fraction
$P\left(m_{\star1},q_\star,z\right)$ and the galaxy merger
time $T_{\rm gal-gal}P\left(m_{\star1},q_\star,z\right)$, both
functions of galaxy stellar mass, redshift, and stellar
mass ratio of the pair, $q_\star$:
\begin{equation}
    \label{eq:gpf}
    P\left(m_{\star1},q_\star,z\right)=
    P_0\left(\frac{m_{\star1}}{10^{11}M_\odot}\right)^{\alpha_p}
    (1+z)^{\beta_p}q^{\gamma_p},
\end{equation}
where $\alpha_p=\alpha_{p,0}+\alpha_{p,z}\cdot z$,
$\beta_p=\beta_{p,0}+\beta_{p,z}\cdot z$, and
$\gamma_p=\gamma_{p,0}+\gamma_{p,z}\cdot z$;
\begin{equation}
    \label{eq:gmt}
    T_{\rm gal-gal}\left(m_{\star1},q_\star,z\right)=
    T_0\left(\frac{m_{\star1}}{10^{11}M_\odot/h}\right)^{\alpha_t}
    (1+z)^{\beta_t}q^{\gamma_t},
\end{equation}
where $\alpha_t=\alpha_{t,0}+\alpha_{t,z}\cdot z$,
$\beta_t=\beta_{t,0}+\beta_{t,z}\cdot z$, and
$\gamma_t=\gamma_{t,0}+\gamma_{t,z}\cdot z$.

%----------------------------------------------------------------

\begin{appendix}
\section{Fixed population parameters}
\label{app:fixedpars}
In Table \ref{tab:fixedvals} we list the parameters that during
the creation of the SMBH binary populations have been kept fixed
to the same values used in \citet{Agazie23b}.
\begin{table}[hb]
    \centering
    \begin{tabular}{c|c}
    Parameter & Value \\
    \hline
    $\psi_z$ & -0.60 \\
    $m_{\psi,0}$ & +0.11 \\
    $\alpha_{\psi,0}$ & -1.21 \\
    $\alpha_{\psi,z}$ & -0.03 \\
    \hline
    $P_0$ & +0.033 \\
    $\alpha_{p,0}$ & 0.0 \\
    $\alpha_{p,z}$ & 0.0 \\
    $\beta_{p,0}$ & 1.0 \\
    $\beta_{p,z}$ & 0.0 \\
    $\gamma_{p,0}$ & 0.0 \\
    $\gamma_{p,z}$ & 0.0 \\
    \hline
    $T_0$ & 0.5 Gyr \\
    $\alpha_{t,0}$ & 0.0 \\
    $\alpha_{t,z}$ & 0.0 \\
    $\beta_{t,0}$ & -0.5 \\
    $\beta_{t,z}$ & 0.0 \\
    $\gamma_{t,0}$ & -1.0 \\
    $\gamma_{t,z}$ & 0.0 \\
    \hline
    $\alpha_\mu$ & +1.10 \\
    \hline
    $a_c$ & $+10^2$ pc \\
    $a_{\rm init}$ & $+10^3$ pc \\
    $\nu_{\rm outer}$ & +2.5\\
    \end{tabular}
    \caption{Fiducial values of the parameters that have
    been kept fixed during the creation of the 1,000 SMBH
    binary populations described in \ref{sec:popcreat}.}
    \label{tab:fixedvals}
\end{table}
\end{appendix}

%----------------------------------------------------------------

To put in the results:

Inserire quante binarie sarebbero detectabili
